Synthesizing Brain-Network-Inspired Interconnections for Large-Scale Network-on-Chips

Brain network is a large-scale complex network with scale-free, small-world, and modularity properties, which largely supports this high-efficiency massive system. In this paper, we propose to synthesize brain-network-inspired interconnections for large-scale network-on-chips. Firstly, we propose a method to generate brain-network-inspired topologies with limited scale-free and power-law small-world properties, which have a low total link length and extremely low average hop count approximately proportional to the logarithm of the network size. In addition, given the large-scale applications and the modular topology, we present an application mapping method, including task mapping and deterministic deadlock-free routing, to minimize the power consumption and hop count. Finally, a cycle-accurate simulator BookSim2 is used to validate the architecture performance with different synthetic traffic patterns and large-scale test cases, including real-world communication networks for the graph processing application. Experiments show that, compared with other topologies and methods, the NoC design generated by the proposed method presents significantly lower average hop count and lower average latency. Especially in graph processing applications with a power-law and tightly coupled inter-core communication, the brain-network-inspired NoC has up to 70% lower average hop count and 75% lower average latency than mesh-based NoCs.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations
	       

==> doc/ack.tex <==
%!TEX root = ../main.tex
\begin{acks}
This work was partially supported by the National Key R\&D Program of China under grant No. 2019YFB2204800, National Natural Science Foundation of China (NSFC) under grant Nos. 61874102, 61732020, 61931008, and U19A2074, and Strategic Priority Research Program of Chinese Academy of Sciences under grant No. XDB44000000. The authors would like to thank Information Science Laboratory Center of USTC for the hardware \& software services.

\end{acks}


==> doc/synthesis.tex <==
\section{Topology Generation}
\label{sec:topo-gene}
Our goal is to construct a perfect limited scale-free and small-world properties topology.
%A semi-deterministic growth algorithm\cite{EyuphanConstructing} is proposed to generate a limited scale-free P2P networks.
At the time of topology generation, performance optimization goals include power consumption and latency. The power consumption of the on-chip network mainly includes the power consumption of switches and the leakage power consumption of physical links.
There is no deterministic traffic between nodes in this stage, so we only consider the power consumption of switches and leakage power of links, and we also assume that there is such an extreme case where there is communication between every two nodes.
%Fault tolerance ability for the random failure of components (link or switch) has been the vital and basic embodiment of system reliability \cite{WuAn}. In complex networks, a metric based on the percolation theory is utilized to evaluate the reliability of the network topology by considering the maximal connected subgraphs after the randomly removal of the a certain fraction of nodes or edges.It also applies to the topological reliability assessment of the on-chip network for random failures. Faults in any part of a switch are considered as the case that faults occur in all the links which are connected to the faulty switch. Hence, here all the faults for both links and switches are classified into the model for faulty links.
As above mentioned, the overall performance tradeoffs of topologies can be expressed as
\begin{equation}
\label{eq:obj-topo}
 OBJ=\alpha*\frac{hop_{min}}{hop}+(1-\alpha)*\frac{pow_{min}}{pow}%+\mu*\frac{rel}{rel_{max}}
\end{equation}
where the coefficients $\alpha$ is experience parameters. In $hop$ represents the average minimum hop count among every two node pair and $pow$ denotes power consumption of all switches, respectively. %$rel$ as rough assessment of reliability is the average fraction of nodes that belongs to the maximal connected subgraph when the network with $b$ certain fractions of random faulty links, respectively.
%$rel$ can be shown as $\frac{1}{b}\sum_{j=1}^b{NR_j}$, and $NR_j=n_{mcs}^j/n$. $n_{mcs}^j$ is the number of nodes which are parts of to the maximal connected subgraph when the fraction of faulty links is $p_j$.
%In equation (\ref{eq:obj-topo}),
$hop_{min}$ and $pow_{min}$ are minimum average hop count and minimum switch power consumption over the possible results of all topologies, respectively.

We propose a deterministic growth algorithm which starts with an initial mesh topology and adds the new nodes into the network one by one. The network has $n$ nodes, each with the minimum degree $k$, each link established between this new node and one existing node will increase the total degree of the network by 2, so the average degree of all nodes is $2k$, and the maximum degree (hard cutoff) is $m$. For obeying the limited scale-free property, the degrees distributed ($k\leq i<m$) according to the power law with exponent $\gamma$.
The frequency $f_i$ of nodes with degree $i$ can be written as $n_i/n$. According to the work \cite{BulutConstructing}, it can be rewritten as
\begin{equation}
  f_i=\frac{m-2k}{i^{\gamma}\sum_{j=k}^{m-1} \frac{m-j}{j^{\gamma}}} \quad for\ k\leq i < m
\end{equation}
\begin{equation}
  f_m=1-\sum_{j=k}^{m-1}{f_i}
\end{equation}
So given $m$, $k$, and $\gamma$, we can obtain the final desired degree distribution of the network. For each edge of new joining node, the algorithm decides which degree (of nodes) accepting such edge will minimize the divergence of the resulting degree distribution from the scale-free distribution. The difference of degree-($i+1$) nodes' expected count and current count in the network is shown as
\begin{equation}
\label{eq:difference}
 d(i)=n[i]-score[i]-freq[i]
\end{equation}
where $n[i]$ denotes current node count with degree-($i+1$), $score[i]$ presents the current expected count of degree-($i+1$) nodes at a given node count, and $freq[i]=f[i]/k$ is the expected increment in degree-($i+1$) node count with only one edge addition to a new node. If the new link is connected to the existing node with degree-($i+1$), the sum of absolute difference of all degrees can be computed as
\begin{equation}
\label{eq:sum-difference}
 D(i)=(|d(i)+1|+|d(i-1)-1|)-(|d(i)|+|d(i-1)|)
\end{equation}
Therefore, select the node degree that minimizes the sum value to adhere the scale-free distribution as much as possible. After that, the new node can select any node with such degree to connect, so as to further satisfy small-world property (length follow a power law distribution $P(l)$ $\propto$ $l^{-\beta}$, where $\beta$ is the exponent, and $l$ represents the link length computed by Manhattan distance),
%that is, the links between nodes are established following a power law ($P(l)$ $\propto$ $l^{-\beta}$ where, $l$ represents the link length, here it is computed by Euclidean distance, and the exponent $\beta$ also affects the locality and performance of the network),
we establish a new edge, which has the maximum deviation in the expected and actual length distribution, between new joining node and the above existing node.
%has a link which minimizes the difference of all link length among the expected link counts and the current link counts, which is finally selected to connect the new node. %also can be calculate by the equation (\ref{eq:sum-difference}).
\begin{figure}[htbp]
\vspace{-0.2cm}  %调整图片与上文的垂直距离
\setlength{\abovecaptionskip}{1mm}
\setlength{\belowcaptionskip}{-0.3cm}
\small \centering
  \includegraphics[width=4.5cm]{../fig/floorplan.eps}\\
  \caption{On-chip Floorplan.}
  \label{fig:floorplan}
\end{figure}

The design flow is as follows:

1. The floorplan is same with TrueNorth chip which consists of a 2-D grid of 64$\times$64 tiles ($n=4096$) and occupies 4.3 ${cm}^2$ in die area. The Manhattan distance of links is in the range $[1, 126]$. Each link represents a bidirectional physical links.

2. The interconnection starts with a 4$\times$4 initial mesh topology consists of black tiles and blue edges at the center of the chip plane as shown in Figure \ref{fig:floorplan}. The coordinates of some nodes are shown in nearby square brackets.

3. In order to construct as many short edges as possible, the remaining nodes are added to the network in order from near to far from the initial network (that is, by fill color from dark to light) until all nodes have been added. Since the average node degree of large-scale mesh network is around 4, the average node degree of the network is consistent with that of the mesh network for a fair comparison, the initial degree of each new node $k$ is 2, that is, two new physical links are established. For given $m$, $\gamma$, and $\beta$, update the node count, and calculate degree distribution differences and link distribution differences following (\ref{eq:difference}) before each new link establishment of new nodes. A link is established to connect the new node with the existing node which makes the network more adherent to the scale-free and small-world properties.

4. We build the brain-inspired topology using the above steps for given parameters $\gamma$ and $\beta$, then evaluate the performance of the network.
Consequently, we vary $\gamma$ and $\beta$ within a certain range and determine the optimum brain-inspired topology for each $\gamma$ and $\beta$ using our design flow.
Finally to choose the optimum value of $\gamma$ and $\beta$, we consider the particular network configuration that maximizes $OBJ$.
%The simulation results will be shown in Section \ref{sec:experiment}.


